Frappe: Understanding the Usage and Perception of Mobile App Recommendations In-The-Wild

This paper describes a real world deployment of a context-aware mobile app recommender system (RS) called Frappe. Utilizing a hybrid-approach, we conducted a large-scale app market deployment with 1000 Android users combined with a small-scale local user study involving 33 users. The resulting usage logs and subjective feedback enabled us to gather key insights into (1) context-dependent app usage and (2) the perceptions and experiences of end-users while interacting with context-aware mobile app recommendations. While Frappe performs very well based on usage-centric evaluation metrics insights from the small-scale study reveal some negative user experiences. Our results point to a number of actionable lessons learned specifically related to designing, deploying and evaluating mobile context-aware RS in-the-wild with real users.

==> methodology.tex <==
%!TEX root =  iuiFrappe.tex
\section{Studying Frapp\'e In-The-Wild}
Recently many researchers have begun to explore the use of app markets like Google Play as a means of recruiting participants and running large-scale mobile user studies in-the-wild \cite{McMillan:2010,Niels:2011}. While this approach offers a number of benefits, in particular related to the amount of quantitative usage data collected, such studies tend to lack qualitative insights. In consequence, researchers in the mobile HCI community have proposed \emph{hybrid} approaches where mobile applications are evaluated both globally via large-scale app market deployments and concurrently in a smaller-scale, local deployments \cite{Morrison:2012}. Such approaches lead to richer insights. We opted to evaluate Frapp\'e using a similar approach which involved: (a) releasing the Frapp\'e app globally via Google Play to attract a large user-base enabling us to gather interesting usage statistics; and (b) concurrently running a smaller-scale local trial in the UK with 33 participants enabling us to gather insights about participant experiences with the recommendations provided. In the following sections we describe each study in more detail. 

\subsection{Large-Scale Study via Google Play}
\begin{figure}[h!]
 \centering
  \includegraphics[width=0.98\linewidth]{img/map}
 \caption{Distribution of downloads around world. \label{fig:map}}
 \end{figure}

 
Frapp\'e was deployed in the Android Market on the February 15th, 2013. We actively advertised the
app among our friends, colleagues and in online social forums such as Reddit. In this paper
we report the results derived from the data collected during a 2 month period from February 15th, 2013 - April 22nd, 2013. 
In total we collected approx. 351K data tuples in the form of $user \times item \times context \times app~usage~count$, where possible values of contexts are
listed in Table~\ref{tab:inputs}. The recommendation model was trained using this data.
\nuria{add details on how many users, usage statistics, avg number of apps installed before using frappe, avg number of apps installed because of frappe,etc...}


The collected data was generated from 340 different types of Android user agents. The distribution of user locations is
shown in Figure~\ref{fig:map}. We had users from 37 countries:
41\% of the user base came from the USA, 13\% from UK, 10\% from Spain, 9\% from Australia, 6\% from Canada,
3\% from Germany and 1.5\% from France. Note that majority of users are from English speaking countries. We also observed the primary language of the recorded apps. Not surprisingly, 91\% of apps are
in English. These are followed by 1.1\% in Chinese , 1.1\% in Spanish and 0.8\% in German. In-depth analysis of the data can be found in the Results Section.
All Frapp\'e users granted permission to share the anonymized app usage data to the research community for further research \footnote{The URL is anonymized for the submission.}.
\nuria{is this true????}

Given the real-world, large-scale nature of the dataset coupled with the richness of the contextual
 factors recorded, we believe that this dataset could be of great benefit to the CARS community and hope it will enable significant advances in CARS research.

\subsection{Small-Scale Local Study}
In this section we describe a 3-week local field study of Frapp\'e with 33 Android users.

\subsubsection{Participants}
Using an external recruitment company based in the UK, we recruited a diverse group of active Android users.
We define an active Android user as a user who has at least five mobile apps installed on their phone and who uses at least one of these apps once per week.
 Participants were required to own a smartphone running Android OS version 2.2 or higher. 
We recruited 33 participants in total, 21 male and 12 female with varied age ranges: 4 participants were between 18-24, 11 participants were between 25-30, 6 participants were between 31-34, while the remaining 12 participants ranged in age between 35-44. 80\% of participants had 10 or more apps installed, while the remaining 20\% of users had 5-9 apps installed.

\subsubsection{Procedure}
\begin{table*}[t]
\small
\begin{tabular}{lll | lll | lll}
Application & Category & \#\textbf{Installed} & Application & Category & \#\textbf{Viewed} & Application & Category & \#\textbf{Used}\\
\hline
Time Lapse		& Photo	&	25		& Flipboard		& News		& 103	& Chrome		& Browser		& 170K\\
Bubble Shooter 	& Game	&	11		& Expedia Hotels	& Travel		& 49		& Gmail		& Email		& 145K\\
Pocket			& News	&	11		& Time Lapse		& Photo		& 49		& WhatsApp	& Messenger	& 136K \\
Bridge the Wall		& Game	&	10		& Bubble Shooter	& Game		& 48		& Facebook	& Social		& 123K\\
Clean Master		& Tool	&	9		& Firefox			& Browser		& 44		&GO Launcher EX	& Launcher		& 94K\\
\end{tabular}
\caption{Most installed v.s. viewed v.s. used applications. \label{tab:used}}
\end{table*}

We used an moderated online community forum to gather subjective insights from our participants. This online qualitative research approach offers a number of compelling advantages: First, online communities run over a prolonged period of time which allows in-depth interaction and collaboration, thus enabling researchers to review and probe topics in more detail and refine questions as the study progresses. Given that the duration of participant interaction with the researchers in an online community is typically longer than in face-to-face methods, this approach can lead to more qualitative insights and richer information. Second, online communities are more cost effective than face-to-face discussions.

Participants were asked to install the Frapp\'e application on their mobile phone and to use it for a period of 3-weeks. During that time participants accessed a closed, online community forum each evening to answer specific questions about their experiences with Frapp\'e. A new topic was posted to the forum 6 out of 7 days per week (\emph{i.e.} everyday except Sundays) by a moderator over the study period. Each topic comprised of a set of sub-questions or tasks. Topics included: 

\begin{enumerate}
\item The installation, usability, functionality, ease of use and look and feel of the application; 
\setlength{\parskip}{0pt}
\item The perceived value and/or drawbacks of the app both initially and after prolonged use; 
\setlength{\parskip}{0pt}
\item The quality, relevance and suitability of the recommendations provided; 
\setlength{\parskip}{0pt}
\item Their understanding of context, their experiences and perceptions in receiving context-aware recommendations and their understanding of the explanations that Frapp\'e provided to them; 
\setlength{\parskip}{0pt}
\item Their use of Frapp\'e in different places and situations and the relevance of recommendations in various contextual settings; and finally
\setlength{\parskip}{0pt}
\item Their attitudes towards control, preference settings, privacy and security.
\end{enumerate}

Participant responses were moderated and if more detail was required or responses were unclear, the moderator could probe participants in more detail. 
Participants were able to see the responses of fellow participants and were also free to engage in group-based discussions should they desire. 
Even though this feature could have led to some biases in their answers, it was not the case in our experience.  
At the end of each day, all forum responses were analyzed and underlying themes were identified. In this way findings from each day could feed into the questioning for the following day. This iterative approach was very beneficial and enabled us to gather a rich set of subjective insights (see Results section). 
